Physiological accuracy in simulating refractory cardiac tissue: the volume-averaged bidomain model vs. the cell-based EMI model

The refractory period of cardiac tissue can be quantitatively described using strength-interval (SI) curves. The information captured in SI curves is pertinent to the design of anti-arrhythmic devices including pacemakers and implantable cardioverter defibrillators. As computational cardiac modelling becomes more prevalent, it is feasible to consider the generation of computationally derived SI curves as a supplement or precursor to curves that are experimentally derived. It is beneficial, therefore, to examine the profiles of the SI curves produced by different cardiac tissue models to determine whether some models capture the refractory period more accurately than others. In this study, we compare the unipolar SI curves of two tissue models: the current state-of-the-art bidomain model and the recently developed extracellular-membrane-intracellular (EMI) model. The EMI model's resolution of individual cell structure makes it a more detailed model than the bidomain model, which forgoes the structure of individual cardiac cells in favour of treating them homogeneously as a continuum. We find that the resulting SI curves elucidate differences between the models, including that the behaviour of the EMI model is noticeably closer to the refractory behaviour of experimental data compared to that of the bidomain model. These results hold implications for future computational pacemaker simulations and shed light on the predicted refractory properties of cardiac tissue from each model.

==> conclusion.tex <==
\subsection*{Conclusion}
For many years, the homogenization approach of the bidomain model has been the accepted technique for simulations in the field of cardiac modelling. Work with this model has made great strides; however, its simplified approach has shortcomings, which may potentially be addressed with more detailed models and greater computing power. 

In this study, we performed a comparative analysis of the bidomain and EMI models in the context of strength-interval curves and the refractory period of cardiac tissue. The aim of the analysis was to identify and explore any advantages of the detailed but computationally expensive EMI model in relation to the less detailed and less expensive bidomain model. %
In carrying out the study, we uncovered noticeable differences between the two models. These differences include the EMI model having a strength-interval curve that is closer to experimental data and a longer relative refractory period than the bidomain model. Although further analysis is needed before direct conclusions are drawn, the present findings are indicators of areas that are worth deeper exploration. Such areas include determining whether the EMI model is better suited than the bidomain model for studying refractoriness, as well as what the factors are that influence SI curves. These areas hold implications for our understanding of the refractory period of cardiac cells and for the design of pacing devices, especially in the shift toward integrating computational tools into these fields of research. 
